Unconfused ultraconservative multiclass algorithms

We tackle the problem of learning linear classifiers from noisy datasets in a multiclass setting. The two-class version of this problem was studied a few years ago where the proposed approaches to combat the noise revolve around a Per-ceptron learning scheme fed with peculiar examples computed through a weighted average of points from the noisy training set. We propose to build upon these approaches and we introduce a new algorithm called UMA (for Unconfused Multiclass additive Algorithm) which may be seen as a generalization to the multiclass setting of the previous approaches. In order to characterize the noise we use the confusion matrix as a multiclass extension of the classification noise studied in the aforemen-tioned literature. Theoretically well-founded, UMA furthermore displays very good empirical noise robustness, as evidenced by numerical simulations conducted on both synthetic and real data.

==> changes.tex <==
%!TEX root=unconfused.tex
\section{Response to Reviews}

\subsection{Preamble}
Once again we would like to thanks the reviewers and the editors for their very
thorough examination of our paper. The relevance of their proposed changes and
remarks undoubtly helped us a lot to improve the overall quality of this paper.
We will give the detail of our responses below. As usual, our comment are tagged
with the command 'ans\{\}'.

\subsection{Response to editors}

{\em
COMMENTS FOR THE AUTHOR:

Editor: There seems to be still a lot of minor issues as pointed out by Reviewer
$3$ and $4$. Please fix.
I apologise for the delay in getting these reviews back to you. There was a mix-up in the paper management system.
}

\ans{We have made our best to fix all of those minor issues. Relevant details
and comments are below.}

\subsection{Response to reviewers}

{\em
Reviewer $1$: The revision has addressed all my concerns, and therefore I
recommend accepting this paper for publication.


Reviewer $3$: 

[\ldots]

DETAILED COMMENTS:

Thank you for your responses, and for the adjustments to the paper. The current
presentation is more clear to me, and the content of the text has certainly
improved.

The editor and Reviewer 1 have suggested clarifying the meaning of $\alpha$.
Have you considered the impact of having $\alpha = 0$ on convergence results
(via the convergence analysis of the perceptron)? This might help explain why
this choice of $\alpha$ worked in practice. Also, it seems to me that the risk
of choosing $\alpha = 0$ is that you might be wasting computation with $z_{pq}$
where you do not really make a mistake; does this occur in practice?

\ans{The introduction of $\alpha$ is dictated by the possible deviation of
$z_{pq}$ from its expected value $\mu^p_q$. In practice, having $\alpha = 0$ not
only implies that we may be wasting computation but also that we may erroneously infer
the true class of $z_{pq}$ leading to unwanted updates and/or update
vectors that are not linearly separable.}

I think the way you generate the confusion matrices in Section 4.1 can be
improved. It seems to me that the fluctuations in Figure 1(b) are due to
fluctuations in the eigenvalues and changes in the eigenvectors. My suggestion
is for you to try an additional setup: fix the eigenvectors of the reference
matrix and perturb its eigenvalues. It would be interesting to see
perturbations in the smallest eigenvalue (by pushing it close to zero), and in all eigenvalues.

The results in Figure 1(b) suggest that the algorithm is not very stable in the
sense that small perturbations to some coordinates of the confusion matrix may
cause the confusion rate to (locally) go up fast. A brief comment from the authors on this would be interesting.

I am a bit puzzled to the meaning of the numbers reported in Section 4.1. In my
opinion you should feed enough data to UMA to learn the true concept when given
the true confusion matrix. This would allow you to better isolate the effect of
perturbations to the confusion matrix.

I have the impression from the theoretical results that UMA performs better
when you provide only confused data (that is, when you confuse even the
labelled data). More precisely, I think that UMA suffers from unconfused data.
Is this the case, or not? If this is the case, how robust is UMA to unconfused
data mixed with confused data? Is there a principled way of confusing the labelled data (besides using a noisy classifier)?

\ans{One of the premises of this work is that labels are generated according to
a class-wise confusion rate. Adding labeled data changes the noise pattern and
introduces errors in the confusion matrix.
A simple workaround is to 'confuse'/contaminate the labelled data according to the confusion matrix.}


REQUIRED CHANGES: DISTINGUISH BETWEEN MINOR AND MAJOR CHANGES THAT NEED TO BE MADE FOR THE PAPER TO BE ACCEPTABLE.

[Minor] Fix the representation across algorithms (e.g., use the same feature
set for the perceptron, UMA and the S3VM) for the experiments with real data.
Not doing so makes the results difficult to interpret, as it is not clear
whether the performance differences are coming from the differences in the
hypotheses spaces, or differences between the methods.

\ans{We have rerun our experiments with the same representation for all
algorithms and updated the paper accordingly. Because the kernel-\pca step is a
constraint specific to \uma, we think our previous results are nonetheless
interesting in order to measure how much errors are induced by this step.
Therefore we decided to keep the error rates for both representations (i.e.
with and without the kernel-\pca step).
}

[Minor] Place the work within context in terms of semi-supervised learning.
Showing that your contributions are, in addition, filling a gap in the
supervised learning literature will emphasize the impact of your contributions.

\ans{One addition of our work to the semi-supervised literature is our bound on
the sample complexity and running time. This has been mentioned more clearly
and emphasized in the introduction.}

[Minor] Fix the few remaining typos and editorial errors (see the end of this
review).

\ans{We have made our best to accomodate all typos (see below for comments).}

[Minor] Compare, in all three datasets, UMA against S3VM with a fixed
(well-chosen) $\mathcal{S}_{\mathrm{conf}}$ size, for various sizes of the
labelled training set, from small sizes to large sizes, and a comparatively
large size of the unlabelled training set.
Fix $u$, the size of the unlabelled data set
$\mathcal{S}_{\mathrm{unlabelled}}$. Fix the size $c$ of
$\mathcal{S}_{\mathrm{conf}}$, having $c \ll u$. Vary the size $l$ of the
labelled data $\mathcal{S}_{\mathrm{labelled}}$ set from $c$ to $u$, following
your experimental protocol for UMA, while training S3VM on
$\mathcal{S}_{\mathrm{labelled}} \cup \mathcal{S}_{\mathrm{unlabelled}}$.
Report the misclassification rate versus $l$ for the UMA and S3VM, on each
dataset. This will allow you to support your claim about UMA's advantage with
few labelled data, and will also inform the reader about how well UMA performs
as the amount of labelled data comes closer to the amount of unlabelled data.

\ans{We added this experiment to our paper and commented it.}

[Minor] Clarify the statement of Proposition 4. The statement here is not as
clear as in Theorem 1. You pass through the data at each iteration, and
generate a point $z_{pq}$ where the algorithm makes a mistake (in the
unconfused data). Your algorithm is operating in a batch scenario, so what does
this limit mean on the number of updates mean? Can you prove that UMA makes at
most that number of updates (before convergence)? This would mean that after
these many updates, you cannot (w.h.p.) construct examples where you make
mistakes, but this does not immediately follow from the online results of
Theorem 1, which is a regret result (you need other results when you pass
multiple times over the data).

\ans{We have reworked the proof of proposition 4 as it seems the confusion came
from here (see the changes for more details). We also added a discussion on how
one can easily turn \uma into an online algorithm at the cost of a much larger
sample complexity. We think that, beyond its technical significance, this
discussion could help the reader to understand the underlying mechanism of
\uma.}

ADDITIONAL CHANGES, FUTURE WORK

No changes in this section are mandatory. Here are some things you could try out, that might improve the understanding of UMA.

Report the performance of SVM on the "subdatasets" 'y', 'conf' and 'full' in Table 1.

Evaluate UMA, in addition, under the following experimental protocol:
(i) Construct the small, balanced dataset as in your original protocol (call it
$\mathcal{S}_{\mathrm{small}}$). Construct a separate $\mathcal{S}_{\mathrm{conf}}$ in the same way.
(ii) Run SVM on $\mathcal{S}_{\mathrm{small}}$ (call the result $h$).
(iii) Estimate the confusion matrix of $h$ on $\mathcal{S}_{\mathrm{conf}}$ dataset.
(iv) Label the $\mathcal{S}$ with $h$.
(v) Run UMA on the labelled $\mathcal{S}$.
The reason I am suggesting this protocol is based on my belief that SVM is
better than the perceptron. When this is indeed the case, you should be using
it when you can, and you should see the performance of UMA improve. This
protocol can (and should) be improved, so that you can compare unconfusion with
the way S3VM imputes labels on the unlabelled data.
If the performance degrades, it will be interesting to know why.

It would be informative to see the performance of UMA in a favorable scenario
as well. With your synthetic data, perform the following experiment:
(i) Pick an integer $M$.
(i) Construct a labelled sample $\mathcal{S}$ of size $m$ and an unlabelled
sample $\mathcal{S}^{'}$ of size $m' = M - m$.
(ii) Run SVM on $\mathcal{S}$ (call the result $h$).
(iii) Compute the confusion matrix of $h$ with very high precision, using as much data as needed.
(iv) Use $h$ to relabel $\mathcal{S}$ and to label $\mathcal{S}^{''}$.
(v) Run UMA with the high-precision confusion matrix on the relabeled and labeled sets together.
Measure the misclassification rate. The comparison should be for various values of $m$, and fixed $M$, against S3VM.
This protocol has the advantage that the confusion matrix is generated more
closely to your "target scenario". I also think relabeling makes sense because
you should not mix confused and not confused data together if UMA expects confused data.

You can also run a modified of the above, which will be affected by how you generate the confusion matrix:
(i) Generate $\mathcal{C}$.
(ii) Generate a dataset $\mathcal{S}$.
(iii) Confuse the data in $\mathcal{S}$ using $\mathcal{C}$.
(iv) Run UMA using $\mathcal{C}$ on the confused $\mathcal{S}$.
Measure the misclassification rate. This is a sanity check, to understand
whether UMA is effective at unconfusing, but step (i) should be done with care.

Increase the number of datasets in which you run your experiments: you should
have enough datasets where UMA can perform well, with a good understanding of
why it works well on these datasets. This should include some synthetic data
where helpful characteristics are prominent. You should also include datasets
where UMA fails (possibly synthetic) -- but where competing methods do not --, where the harmful characteristics are prominent.
Designing synthetic data as above can be challenging, but it will certainly
deepen the understanding of UMA, and help inform the reader about when to use it.

\ans{The discussion here is very fruitful and these changes and additionnal
experiments are indeed interesting. However, we feel like these changes require
a very thorough study of the new results they imply and therefore fall beyond
the scope of a minor revision. Nonetheless, we highly value this feedback and
surely consider including these experiments on our future works on the subject.}

TYPOS

Please consider the following editorial changes as well (where [a:b] indicates
page a, line b, and [a:b-c], page a, lines b to c). Some of these are stylistic suggestions.

$[1:20]$ Remove the citations from the abstract. \\
$[1:36]$ These paragraph headings in the introduction are good and helpful to
the reader. \\
$[1:40]$ \dots, Q \\
$[2:6]$ Italicize i.e., e.g., etc. \\
$[2:8]$ to provide the \\
$[2:12]$ Use $C$ instead of $\mathcal{C}$. \\
$[2:12]$ Put $\mathcal{C}_{pt(x)}$ on the left-hand side. \\
$[2:22]$ Some readers are very sensitive about how you use "very" -- using this
word prompts some readers to take whatever you write afterward literally.\\
$[2:27]$ provided that:\\
$[2:44]$ to realistic\\
$[2:50]$ I would say that $f$ makes mistakes evenly over the class regions.\\
$[3:2]$ Cite the ACML paper -- "an extended version of [...]."\\
$[3:12]$ data if some\\
$[3:15]$ massive amounts\\
$[3:23]$ Use alternatives to "online", e.g., "iterative" (as opposed to "batch").
"Online" may these days be mistaken with with the online learning setting.\\
$[3:38]$ losses, were\\
$[3:42]$ and it makes\\
$[4:9]$ in the PAC literature\\
$[4:26]$ The linear classifier\\
$[4:27]$ with respect to the concept $c$\\
$[4:31]$ $\theta \geq 0$\\
$[4:38]$ ($\| \cdot \|_F$ denotes the Frobenius norm)\\
$[5:8]$ of $Y$ is the same for all $x \in X$ and its conditional\\
$[5:17]$ The noise process $Y$.\\
$[5:17]$ a) aggressive\\
$[5:19]$ b) regular \\
$[5:47]$ is a research \\
$[6:2]$ Maybe these subsection headings should be bold.\\
$[6:7]$ of $f$ is as small\\
$[7:3]$ $\mathcal{S}_{\mathrm{true}} = \{ (x_i, t(x_i)) \}_{i=1}^n$\\
$[7:29]$ $\mathcal{S}_{\mathrm{true}}$\\
$[7:46]$ Algorithm 2 the\\
$[8:7]$ $\backslash set$\\
$[8:9]$ $\backslash alpha$\\
$[8:49]$ steps 4 through\\
$[9:1]$ $q$ with high probability\\
$[10:17]$ Move this remark to the paragraph before the proposition.\\
$[10:22]$ $p$; $\mu_p^q$\\
$[10:33]$ with (10) and the linearity\\
$[11:4]$ $1 - \delta$ for any\\
$[11:17]$ $\alpha = \varepsilon$\\
$[11:24]$ Idem.\\
$[11:24]$ just says\\
$[11:28]$ that the parameter\\
$[11:44]$ Under Assumptions\\
$[12:50]$ class\\
$[13:2]$ an algorithm for minimizing the confusion risk\\
$[13:29]$ axes\\
$[13:46]$ This matrix looks like a recall matrix.\\
$[13:50]$ $\hat{y}_i = p$\\
$[13:51]$ I would suggest eliminating the diagonal here, rather than mentioning
later that it is eliminated.\\
$[14:10]$ has norm $1$\\
$[14:13]$ to the decision\\
$[14:16]$ with a small\\
$[14:13-16]$ Please make this paragraph more clear.\\
$[14:25]$ algorithm with various \\
$[15:20]$ I think it would be interesting to see $\| \cdot \|_{\infty,\infty}$ as
well. 
\ans{see 15:15 below.} \\
$[15:34]$ dataset, and then each\\
$[15:49]$ performance degrades as\\
$[15:15]$ Do the numbers have any specific meaning? Is the scale between the worst
and best confusion rates significant?
\ans{We have reworked the confusion rate for it to be between $0$ and $1$ (see
the relevant section in the paper). This should bring more interpretability of
our result and easier comparison with the error rate. We also discussed adding
more performance measures based on $\Conf$ but we came to the conclusion it
would negatively impact the overall readability of the experimental section now
that we have revised the formula of the confusion rate.} \\
$[15:15]$ How did you ensure that the perceptron "converged"? Did you follow
Proposition 4? 
\ans{We clarified this matter (see Section 4.1, at the end of 'robustness to
noise'). We basically use \uma with the identity matrix.}\\
$[15:26]$ What is your rough classifier? The perceptron? Why not an SVM? $[15:39]$
limitations of UMA 
\ans{Added a footnote on this. We use \uma with the identity matrix (i.e. a
perceptron) for the sake of selfcontainedness}\\
$[15:40]$ What about an $f_{\mathrm{SVM}}$?
\ans{The focus in this section is to investigate the improvements induced by
the use of the confusion matrix, for this purpose a regular perceptron is
much more fit to the task because of its connection with \uma. The \SSVM is
mentioned as an exemple of Semi-supervised algorithm only. Notably, including an
$f_{\mathrm{SVM}}$ would require careful optimization of kernel and model
hyperparameters which is not currently the focus of our experimental section.}\\
$[16:2]$ data as UMA but we use\\
$[16:7]$ problems and\\
$[19:12]$ across datasets which is clearly\\
$[19:18]$ tends to confirm this, particularly ... (add citations for this claim)
\ans{This is no longer needed as this section has been reworked (see the
required change about data representation above)}\\
$[19:34]$ accurate estimate\\
$[20:14]$ Give a more informative label for the $x$ axis\\
$[20:14]$ Generate a ps/pdf image, as your figures are aliased. (Also ensure that
the image's fonts are of correct Type, like Type 1.)
\ans{All figures have been entirely remade and are much more clear now}\\
 $[20:50]$ aim to explore\\
$[21:45]$ core ideas\\
$[21:50]$ requires learning\\
$[21:50]$ incur\\
$[22:14]$ simpler tools\\
$[23]$ Why is your appendix in smaller font?\\
$[23:45]$ fixed pair $(p,q)$\\
$[24:4]$ Check the dashes -- and the spacing around them throughout the text.\\
$[24:5]$ This approach has connections to preference learning and ranking, where
examples are of a single class. Also, why not use $\ell^f(x)$, if the label is
disregarded? \\
$[24:14]$ remove $\times$ \\
$[24:18]$ Namely:\\
$[25:31]$ realizations\\
$[25:36]$ together yields the result\\
$[25:38]$ Recall that\\
$[25:48]$ I think you also need to argue that a covering of $\mathcal{F}_{pq}$
can be used to show concentration over $\widehat{\mathcal{F}}_{pq}$, otherwise
you will have to run into a complicated argument about how to make the result
hold for all $\mathcal{F}_{pq}$ (each constructed for a different
$\mathcal{A}^\alpha_p$).\\


Reviewer $4$: A good revision.

Corrections
===========

page 2 line 7:  use ";" after "procedure"\\
page 3 line 15: "to handle *a* massive"\\
page 3 line 17: "," after "analysis of it"\\
page 3 line 26: "that *a* sample"\\
page 3 line 36: "tackle" to "tackling"\\
page 3 line 50: don't use "evidence" as a verb\\
page 7 line 49: by convention, use plural "assumptions"\\
page 12 line 50 to page 13 line 1:  "account classes distribution"\\
        I couldn't figure out the grammar\\
page 13 line 9:  change "being" to "is"\\
page 14 line 25:  change "to" to "with"\\
text on graphs in figure 1 are way too small; check others too!\\
page 18 line 24:  "that we do not have conducted" ?\\
    maybe "that we have not conducted"\\
page 18 line 25:  change "others" to "other"\\
page 19 line 18:  give references for literature mentioned\\
page 19 line 18:  change "kernel" to "kernels"\\
page 20 lines 36-38:  didn't understand the sentence\\
page 21 line 42:  change "label" to "labels"\\
page 21 line 45:  change "idea" to "ideas"\\
page 21 line 50: change "incurs" to "incur"\\
page 22 line 4: change "avoid" to "avoids"\\
page 22 line 6:  change "problem" to "problems"\\
page 22 line 6:  "to *a* bi-class mapping"\\
page 22 line 7:  "and *a* convergence rate"\\
page 22 line 14: "of *a* multiclass"\\
page 22 line 18:  change "thanks" to "due"\\

Capitals need fixing in references:  ERM, Monte Carlo, Nystr\"om, MKPM.\\
}

\iffalse
\section{Response to Reviewers}

\subsection{Preamble}
First of all, we would like to thank the reviewers and the editor for their 
insightful and very constructive comments. We tried and made our best to 
take all of them into account. The details of the responses we made to the 
questions pointed out by the reviewers are given below. In the following, our
comments are denoted by the '\ans{}' command.

\subsection{Responses to editor}
{\em
All authors mention a number of problems with typos, etc.
Please correct all these and go through the paper again to
look for more.  Chances are, there are more still.
}


\ans{We have tracked all possible typos according to the feedback of the reviewers and we have made additional passes to spot other potential typos.}


{\em
Reviewer \#1 says:  The influence of the value of $\alpha$ still seems slightly unclear.
 It will be great of some comments can be made on its theoretical and practical implications.  Please address this.
}

\ans{We have addressed this
 question and we have added the following comment in the text:
\textit{Note that $\alpha$ is needed to offset statistical (im)precision. Indeed, we can
only approximate $\langle\V{w}_p,\xup{pq}\rangle -
\langle\V{w}_k,\xup{pq}\rangle$ in \eqref{eq:zerror} up to a precision of
$\epsilon$. Thus for the result to hold we need to have
$\langle\V{w}_p,\mu_{q}^p\rangle - \langle\V{w}_k,\mu_{q}^p\rangle > \epsilon$
which is obtained from \eqref{eq:muerror} when $\alpha \doteq \epsilon$.
In practice, this just say that the points used in the computation of $\xup{pq}$
are at a distance at least $\alpha$ from any decision boundaries.}}

\ans{\textit{Remark : It is important to understand that parameter $\alpha$
helps us derive sample complexity results by allowing us to retrieve a 
linearly separable training dataset with {\em positive} margin 
from the noisy dataset. The theoretical results we prove hold for any
such $\alpha>0$ parameter and the smaller this parameter, the larger the
sample complexity, i.e., the harder it is for the algorithm to take
advantage of a training data that meet the sample complexity requirements.
In other words, the smaller $\alpha$, the less likely it is for \uma to
succeed; yet, as shown in the experiments, where we use $\alpha=0$, \uma
continues to perform very well.}
}


{\em
Reviewer \#3 says all the assumptions need to be made clear up front (i.e.,  uniform noise given the real class)}
We have recalled the assumptions at the very beginning of the paper, in section 2.
 
 
\ans{ Now assumption 1 (linear separability with margin condition), assumption 2 (knowledge of the confusion matrix),
  and assumption 3 (invertibility of the confusion matrix) are now given up front.}


{\em
Reviewer \#2 makes a number of suggestions, some implicit:
\begin{itemize}
\item Core idea of UMA is underemphasized, and could be better explained intuitively (outside of the proofs and algorithm details).
\item Could you use knowledge of $C$ in other algorithms?
\end{itemize}
}


\ans{ First of all, there do not seems to be a reviewer \#2. Also, these concerns exists in the feedback
provided by Reviewer \#3 while the third review (by reviewer \#4) simply says "\emph{Way outside my area}". 
Anyhow, we have taken them into account as detailed at the end of this document (see : response to reviewer \#4)}


\subsection{Responses to Reviewers}

{ \em
{\bf Reviewer \#1:}

 This paper learns a linear classifier (or kernelized by kernel PCA) for 
multiclass problems when there is noise in the label. 

[\ldots]

It might be worthwhile pointing out that the theoretical results are not to establish the Bayesian 
optimality of the solution, ie not to guarantee the optimal minimization of $R_{error}$ in Section 2.2.  

\ans{We added the following precision on this matter at the end of section
$2.2$ :}

\ans{\textit{
Our goal is thus to learn a relevant matrix $W$ from
$\inputset$ {\em and} the confusion matrix $\confusion$. More precisely, we
achieve risk minimization through classic additive methods and the core of
this work is focused on computing noise-free update points such that the
properties of said methods are unchanged. 
}}

One may also 
want to stress that the result assumes linear separability.

\ans{We added an early mention of the linear separability assumption for for $S_{true}$ in the introduction at the middle of page 2} 

The influence of the value of $\alpha$ still seems slightly unclear.  It will be great of some comments can be made 
on its theoretical and practical implications. 


\ans{A paragraph was added at the beginning of page $11$ about the practical and
theoretical aspects of $\alpha$. (See response to editors)}



There are a number of typos. I list a few here and the author may wish to polish it more.

1. Line -3 on page 2: thorougher -> more thorough
2. Line 7 on page 3: caracterize -> characterize
3. Line -4 on page 3: intput -> input
4. Mid of page 6: implicitely -> implicitly, explicitely -> explicitly
5. Line 2 below Eq 6: achieve an inner product -> achieve a larger inner product


\ans{These typos have been corrected.}




{ \bf Reviewer \#3:}

 1. OPENING REMARKS

In sections 2, 3 and 4 I summarize the paper, and assess its strengths and weaknesses.
In section 5, I give details about my claims in sections 2, 3 and 4 and make some remarks that will hopefully be helpful to the authors.
Section 7 contains the references, and section 8, the typos.

[\ldots]

Assumption (a) has been employed far and wide, but, when I see it, I think that in most of the cases there is no such large-margin 
separation, so it oversimplifies many problems.
I am not against this assumption in your paper, though, because I think your strategy of using assumption (b) on top of (a) is an 
interesting way of tackling certain problems with label noise.
You must make assumption (b) explicit, as it is hidden in eq. (4), and it is essential to your work.


\ans{We added an assumption block at the beginning of page $5$ in order to make assumption $(b)$ more clear. As a consequence, we also
rephrased the text directly following this new assumption. Also, all the
assumptions are now made clear up front in Section $2.1$}


Also, you might have to convince less motivated readers that this is a reasonable assumption for some important practical problems.


\ans{We added the following argument at the beginning of page $5$ to support
this :}

\ans{\textit{
Nonetheless, this setting fits many
real case problems as numerous noising phenomena
can be accurately summarized by a simple confusion matrix. Moreover it has been
proven \cite{blum96polynomialtime} that robustness to classification noise
generalizes robustness to monotonic noise where, for each class, the corruption
rate is a monotonic decreasing function of the distance to the class boundaries.
}}

[\ldots]

Here is my opinion on the invertibility of (c): it may not be a big problem if some matrix is not invertible, but a bigger problem may
 be if the matrix has poor conditioning. My experience with using inverses of matrix estimates lead me to repeatedly derive high-probability 
 bounds that have a factor of $\sqrt{1/v}$ on the bounding term, where $v$ is the smallest eigenvalue of the matrix we are estimating. You could
  add small-enough diagonals to control the conditioning of the estimate of the matrix, but if the matrix itself has poor conditioning, avoiding
   the $\sqrt{1/v}$ becomes quite a challenge.
   
\ans{We added the following discussion about about matrix invertibility at the
end of Section $2.1$.}

\ans{\textit{
Generally speaking, the problems that we are interested in (i.e.
problems where the true classes seems to be recoverable) tend to have
invertible confusion matrix. It is most likely that invertibility is merely a sufficient
condition on $\confusion$ that allows us to establish learnability in the
sequel. Identifying more stringent conditions, which would for instance be
based on the condition number of $\confusion$ is an issue of its own, poses
questions that go beyond the scope of the present paper and that we left for future investigations.
}}

About the algorithm:

It seems as though the novelty in the algorithm consists of two separate ideas:
i) re-weight examples to force the perceptron to make a mistake;
ii) invert to C to bypass the label noise (unconfuse).

[\ldots]

Moreover, we have that $(q^T)C = p^T$ where $p_i = P(t(X) = i)$ and $q_i = P(Y = i)$, so if you think of your problem as a multiclass
 classification problem as defined in (Pires, Sepesvari \& Ghavamzadeh, 2013), for example, you can minimize a multiclass classification
  loss where the cost of attributing class $i$ to an instance with $Y = j$ is $C_{ij}$, and that should allow you to find a classifier that
   performs as well as the true concept $t$.


   \ans{We added a remark after assumption 2 where we mention this slightly
   different problem : }
   
   \ans{\textit{
   Remark : The confusion matrix $\confusion$ should not be mistaken with the matrix
$\tilde{\confusion}$ of general term : $\tilde{\confusion}_{ij} \doteq
\proba_{X\sim\UKDistri_{X|Y=j}}(t(X) = i | Y = j)$. The problem of learning from
a noisy training set and $\tilde{\confusion}$ is a different problem than the
one we aim to solve. Notably $\tilde{\confusion}$ can be used to define
cost-sensitive losses while $\confusion$ does not allow it. Nonetheless, this
second problem is far from trivial and, although very interesting, largely
beyond the scope of this current work.
   }}



5.2 THEORETICAL ANALYSIS

Your theoretical analysis shows that you successfully used the knowledge of C to unconfuse the perceptron algorithm, and you leveraged the use
 of (i) to find a stopping condition.
You have to deal with some technical issues in the appendix (see the last section of this review), but the results there are believable and the
 ones in the main text seem correct to me.

[\ldots]

7. TYPOS AND OTHER REMARKS

The typos will be stated in the imperative to shorten writing, but please take them as style suggestions.

\ans{In the following list, we have commented some suggestion in order to give
clarification on how these precise points have been tackled in our revision.
The remaining suggestions have been directly transcribed.}

p.2 \\
   3: use $X_i$ and $Y_i$, since they are random variables. 
   \ans{We now say plainly that $x_i$ and $y_i$ are realizations of independent
   random variables.} 
   36: how can one use effective semi-supervised learning
   algorithms to be successful in Example 1? 
   \ans{One can directly run a semi-supervised algorithm on $S$ in the case of
   Example 1.
   Indeed, a small part of it ($S_l$) is already labelled while the rest ($S_u$)
   is not. Semi-supervised algorithms are specifically designed to deal with such
   training sets.
   }
   \\
   37: "scenarios where more labeled data cannot be acquired" \\
   49: "which confirm the relevance" \\

p.3 \\
   13: avoid "valiant" in this situation \\
   22: "many advances" \\
   47: should you assume that $\|X\| \leq 1$ holds w.p. 1, instead of $\|X\| =
   1$? \\
   \ans{We moved this after definition $1$ where it makes sense. Indeed, the
   definition of linear classifier we give (i.e. hyperplane passing through the
   origin) allows us to make this assumption without loss of generality. Note
   that the, seemingly, more general setting can be retrieved from this one by
   adding a dimension to the training set.}

p.4 \\
   26: $\| w^* \|_F^2$ \\
   47: "is almost-surely fully summarized"  \\
   \ans{We clarified the point on the direct link between the
   confusion matrix and the noising process.}

p.5 \\
   3: "This noise" or "The noise" \\
   9: $D_{Y|X}$ \\
   44: I disagree that the heart of the procedure is its update scheme.
   \ans{We revised the wording of this specific sentence}  \\

p.6 \\
   27: "implicitly" \\
   28: "explicitly" \\

p.7 \\
   3: "confusion matrix $C$" \\
   7: $\mathcal{A}_p^\alpha$ \\
   9: $\mathcal{A}_p^\alpha = \{ x : x \in S, \langle w_p - w_k, x \rangle >
   \alpha \}$ \\
   15: $\sum_{i=1}^n$ \\
   19: use $M$ instead of $A$. \\
   49: "Theorem 1, which shows the convergence of ultra-" \\
   50: "conservative algorithms, rests" \\

p.8 \\
   38: same as p.7, 9. \\
   50: avoid using subscripts to expectations at all costs, when they mean you are integrating out a certain variable. That creates a lot of confusion.
    I find it reasonable, though, to subscript the expectation to the distribution of a particular random variable, or to indicate the measure you are
     integrating with respect to. \\ 
   
p.10 \\
   48: "This result" \\

p.11 \\
   8: it should be $f(X) \neq t(X)$. \\
   8: the potential dependence of p and q on W is overlooked in eq. (17). \\
   10: "update may lead" \\
   11: when/how can you guarantee that $z_{pq}$ is more reliable? \\
   \ans{We made clear that this section discusses heuristics that are beyond our
   theoretical analysis} 
   18: $\mathbb{I}\{ t(X_i) = q \}\mathbb{I}\{ f_W(X_i) = p \}$
   \\

p.12 \\
   3: "we remark" \\
   47: same as p.11, 18. \\

p.13 \\
   6: "same distribution as the" \\
   19: in experiments, you should never just say "randomly" -- specify the
   underlying distribution. \\
   20: $N = \frac{M - I}{10}$ \\

p.14
   38: "to an ill-conditioned confusion matrix"
   39: "hence removing"

p.15 \\
   10: "inpractical" \\
   10: why do you not empirically evaluate your method in this setting, in which
   the other algorithms are impractical? (Or when there is a labeling budget.)
   \\
   14: "reproducibility we used datasets" 14: but are these datasets suitable
   for evaluating your algorithm empirically? Reproducibility and suitability
   are both essential. \\
      \ans{We added some comments on these matters ($10$, $14$) in the main
      text. (See the last two paragraphs before section $4.2.1$)}
      34: same as
      p.13, 19.
      \\

   
p.16 \\
   19: in no place have you indicated how the performance was measured; from
   the discussion I had to infer that the comparison metric was
   misclassification error. \\
    \ans{We have clarified this up}

p.17 \\
   20: "carries less" \\

p.18 \\
   41: "theoretical guarantees. Therefore they constitute an ideal" \\
   45: rephrase and formalize "we stuck with more classical tools here"
   (last three paragraphs of the conclusion): the text is too casual, so it
   should be rephrased. \\
   \ans{Most of the conclusion have been rephrased and the text is now more formal}

p.20 \\
   21: the loss is not correct. It could be, e.g., $1 - y*f(x)$ if $y \in
   \{-1,1\}$ \\
    22: the loss is Lipschitz over $\mathcal{Y}$; if you use the
   assumption in p.3, 48, along with boundedness of $w$, then you get the
   Lipschitz condition you need for your results, or you need to truncate
   $f(x)$ to be in $[-1,1]$. I suggest constraining the the $w$ underlying
   $\mathcal{F}_{pq}$ to a ball of a certain radius. \\
     \ans{The function is correct but the use of the word "loss" was misleading. We have reworked this part of the proof for better clarity.}
   23: $(d+1)$, instead of $(n+1)$? \\
   30: avoid using $\leq O(...)$. It is better to use $= O(...)$ or, better,
   $\in O(...)$ \\
    37: use conditioning, not subscripts such as $T|T's$ \\
   44: idem \\
   48: I think it should be $\geq$, not $=$ in this line \\

p.21 \\
   6: "Define" (no "Let") \\
   18: conventionally, people use expectation of a random Rademacher variable
   $\sigma$, rather than the explicit summation over  all possible "binary
   numbers" of $m$ bits. \\
   \ans{Added a footnote about this}

p.22: \\
   3: $\mathbb{I}\{ x \in \mathcal{A}^\alpha_p \}$, and the set should be a
   $\|\cdot\|$-ball of radius one, not $\mathbb{R}^d$. \\
   7: $d+1$ \\
   8: "It comes" \\
   10: $\mathbb{I}\{ x \in \mathcal{A}^\alpha_p \}$ \\
   10: the dependency of $z_{pq}$ on a certain $w$ via $\mathcal{A}^\alpha_p$
   may break this proof, so I suggest you make the argument more clear on that
   matter. \ans{We clarified this point.} \\
   21: same as p.20, 30. \\



{\bf Reviewer \#4:} 

Way outside my area.

\ans{Based on the summary provided by the editors, this review seems out of
place. Nonetheless, we have made changes based editor's feedback.
Namely, we have emphasized the core idea behind UMA in the introduction (see
contribution). Moreover, as part of the rephrasing of the conclusion, we have
more clearly separated the core idea from its implementation within the
additive setting. We also added mentions of the adaptability of our approach to
other (non-additive) algorithms.}

}
\fi










==> header.tex <==
% -*- coding: utf-8 -*-
\usepackage{amsmath,amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{bm} %bold math

\usepackage{xspace}
\usepackage{graphicx}
\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{tikz}

\usepackage{algorithm}
\usepackage{algorithmic}

%\RequirePackage{algorithmic}
\RequirePackage{color}

% ajout Ugo
\newcommand\ans[1] {{\textbf{\\ #1 \\}}}
\newcommand\Ugo[1] {\textcolor{blue}{\textbf{UL : #1}}}
\newcommand\Todo[1] {\textcolor{green}{\textbf{TODO : #1}}}
\newcommand\V[1] {\bm{#1}} %vector
\newcommand\Ex[2] {\mathbb{E}_{#1} \left[ #2 \right]} %expectation (long version)
\newcommand\dotProd[2] {\left< {#1} , {#2} \right>}
\newcommand\norm[1] {\Vert {#1} \Vert}
\newcommand\UKDistri{\mathcal{D}}
\newcommand\setA[1]{\mathcal{A}_{#1}}
\newcommand\gammapt[2]{\gamma_{#1}^{\setA{#2}}}
\newcommand\gammalong[2]{\Ex{p(\V{x}_i | t_i = p)}{\V{x}_i}}
\newcommand\mupt[2]{\mu_{#1}^{#2}}
\newcommand\mulong[2]{\Ex{p(\V{x}_i | y_i = p)}{\V{x}_i}}
\newcommand\xup[1]{\V{z}_{#1}}
\newcommand\size[1]{\vert {#1} \vert_S}
\newcommand\fro[1]{\norm{{#1}}_F}
\newcommand\EV[1]{\E{\V{#1}}} %expectation of a vector
\newcommand\E[1]{\widetilde{#1}} %expectation
\renewcommand\H[1]{\widehat{#1}}
\newcommand{\confusion}{C}
\newcommand{\classes}{{\cal Q}}
\newcommand{\change}[2]{\textcolor{red}{\---old : #1\---}\textcolor{cyan}{#2}}
\newcommand{\changeok}[2]{#2}

%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{example}{Example}

\renewcommand{\iff}{\Leftrightarrow}
%\newcommand\Up[1]{\overline{#1}} %'upperline'
%\newcommand\UV[1]{\Up{\V{#1}}} %vector 'upperline'
%\newcommand\Ident{\V{I}} %identity matrix
\newcommand{\uma}{{\tt \normalsize U}{\tt MA}\xspace}
\newcommand{\SSVM}{\text{{\tt S3VM}}\xspace}
\newcommand{\margin}{\theta}
\renewcommand{\algorithmicensure}{{\bf Output:}}
\renewcommand{\algorithmicrequire}{{\bf Input:}}
\newcommand{\uniform}{\mathcal{U}}
\newcommand{\pca}{\text{\tt PCA}\xspace}
\newcommand{\kpca}{\text{\tt KPCA}\xspace}

%%% Theorems, etc
%%%
%%% Comments
\newcommand{\liva}[2]{\textcolor{blue}{#1}\textcolor{magenta}{{\bf\xspace was} #2}}

\newcommand{\ontop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
\newcommand{\indicator}[1]{\mathbb{I}{\left\{ #1 \right\} }}
\DeclareMathOperator*{\argmax}{\text{argmax}\;}
\DeclareMathOperator*{\argmin}{\text{argmin}}

%%% Misc. shortcuts
\def\algo{\mathcal{A}}
\def\inputset{\mathcal{S}}
\def\trainingset{\mathcal{S}}
\def\inputz{\mathcal{Z}}
\def\distribution{D}
\def\proba{\mathbb{P}}
\def\inputspace{\mathcal{X}}
\def\outputspace{\mathcal{Y}}
\def\targetspace{\mathcal{Y}}
\def\productspace{\mathcal{Z}}
\def\proba{\mathbb{P}}
\def\expectation{\mathbb{E}}
\def\realset{\mathbb{R}}
\def\naturalset{\mathbb{N}}
\def\integerset{\mathbb{Z}}
\DeclareMathOperator*{\union}{\cup}
%\newcommand\union{\cup}
\def\inter{\cap}
\def\family{\mathcal{H}}
\def\loss{\ell}
\def\risk{R}
\def\distributions{\mathcal{D}}
\def\rank{\text{rank}}
\def\pac{\xspace{\sc Pac}}
\def\pefc{\text{\sc Pefc}}
\def\auc{\text{\sc Auc}\xspace}
\def\roc{\text{\sc Roc}\xspace}
\def\sign{\text{sign}}
\def\np{\text{\sc Np}}
\def\normal{\mathcal{N}}
\def\identity{I}
\def\iid{{\sc IID}\xspace}
\def\hypothesis{H}
\def\hypotheses{\mathcal{H}}
\def\variance{\mathbb{V}}
\def\test{\text{test}}
%%% Bold font
\def\bfell{\boldsymbol{\ell}}
\def\bfzero{\boldsymbol{0}}
\def\bfx{\boldsymbol{x}}
\def\bfa{\boldsymbol{a}}
\def\bfz{\boldsymbol{z}}
\def\bfh{\boldsymbol{h}}
\def\bfZ{\boldsymbol{Z}}
\def\bfz{\boldsymbol{z}}
\def\bfD{\boldsymbol{D}}
\def\bfC{\boldsymbol{C}}
\def\bfP{\boldsymbol{P}}
\def\bfQ{\boldsymbol{Q}}
\def\bfS{\boldsymbol{S}}
\def\bfs{\boldsymbol{s}}
\def\bfX{\boldsymbol{X}}
\def\bfY{\boldsymbol{Y}}
\def\bfu{\boldsymbol{u}}
\def\bfv{\boldsymbol{v}}
\def\bfw{\boldsymbol{w}}
\def\bfy{\boldsymbol{y}}
\def\bfpi{\boldsymbol{\pi}}
\def\bfalpha{\boldsymbol{\alpha}}
\def\bfmu{\boldsymbol{\mu}}
%Ugo
\def\UCPA{\text{UCPA}}
\def\UCPAlong{\textit{UnConfused Passive Aggressive}}
\def\UMA{\text{UMA~}}
\def\PA{\text{PA}}
\def\PAlong{\textit{Passive Aggressive}}
\def\Pdim{\text{Pdim}}
%\def\margin{m}
\def\Conf{\confusion}
\def\dist{\text{dist}}
\def\terror{\text{error}}
\def\tconf{\text{conf}}
\def\tcorrect{\text{corr}}
\def\tmixt{\text{mixt}}
\def\tother{\text{other}}
\def\bigE{\mathcal{E}}
\def\bigG{\mathcal{G}}
\def\bigC{\mathcal{C}}
\def\bigO{\mathcal{O}}
\def\bigH{\mathcal{H}}
\def\bigF{\mathcal{F}}
\def\bigI{\mathcal{I}}
\def\bigJ{\mathcal{J}}
\def\bigN{\mathcal{N}}
\def\bigM{\mathcal{M}}
\def\diag{\text{diag}}
\def\err{\text{err}}

%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SMALL EQUATIONS

\usepackage{exscale}
\makeatletter
\newenvironment{equationsize}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \equation
}{\endequation \ignorespacesafterend} 
\makeatother

\makeatletter
\newenvironment{equationsize*}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \equation
}{\nonumber\endequation \ignorespacesafterend} 
\makeatother


\makeatletter
\newenvironment{alignsize}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \align
}{\endalign \ignorespacesafterend} 
\makeatother

\makeatletter
\newenvironment{alignsize*}[1]{% 
  \skip@=\baselineskip 
  #1% 
  \baselineskip=\skip@ 
  \start@align\@ne\st@rredtrue\m@ne
}{\endalign\ignorespacesafterend} 
\makeatother

%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "article"
%%% End: 

